Fast radio bursts at the dawn of the 2020s

Since the discovery of the first fast radio burst (FRB) in 2007, and their confirmation as an abundant extragalactic population in 2013, the study of these sources has expanded at an incredible rate. In our 2019 review on the subject we presented a growing, but still mysterious, population of FRBs -- 60 unique sources, 2 repeating FRBs, and only 1 identified host galaxy. However, in only a few short years new observations and discoveries have given us a wealth of information about these sources. The total FRB population now stands at over 600 published sources, 24 repeaters, and 19 host galaxies. Higher time resolution data, sustained monitoring, and precision localisations have given us insight into repeaters, host galaxies, burst morphology, source activity, progenitor models, and the use of FRBs as cosmological probes. The recent detection of a bright FRB-like burst from the Galactic magnetar SGR~1935+2154 provides an important link between FRBs and magnetars. There also continue to be surprising discoveries, like periodic modulation of activity from repeaters and the localisation of one FRB source to a relatively nearby globular cluster associated with the M81 galaxy. In this review, we summarise the exciting observational results from the past few years. We also highlight their impact on our understanding of the FRB population and proposed progenitor models. We build on the introduction to FRBs in our earlier review, update our readers on recent results, and discuss interesting avenues for exploration as the field enters a new regime where hundreds to thousands of new FRBs will be discovered and reported each year.

==> junk.tex <==

%\section{Figure ideas}


%\includegraphics[width=\linewidth]{Figures/speclum.pdf}

%\includegraphics[width=\linewidth]{Figures/Kumar_Parkes_UWL.png}

%\includegraphics[width=\linewidth]{Figures/National_Geo_galaxies.jpg}



%\includegraphics[width=\linewidth]{Figures/Localizations_overview_v2.png}

%\includegraphics[width=\linewidth]{Figures/repeater_chart.pdf}

%\includegraphics[width=\linewidth]{Figures/2x2_combined_figure_2.pdf}

\begin{comment}

\section{Weekly meeting notes}

\textbf{Friday 14 August}
\begin{itemize}
    \item We seem to be in basic agreement with the editors about what we want the review to look like. They would like us to call it "Fast Radio Bursts: an Addendum" and tack it on with the previous review, which I'm happy to do. As for length, Luigina said that 25-30 pages sounds fine to her. So we will continue to work off of our current outline.

\item We mostly talked about what figures we'd like for the review. 
\item I asked my research group for what diagrams they'd like to see and I suggest each of us does the same. Ask others what sort of figures they would like for their talk slides
\item Planning to make the following figures at least:
\begin{itemize}
   \item Macquart relation (DM v z) - make our own since theirs doesn't have R3 or the new VLA burst. Also the idea of plotting the actual measured total DM and then having downard error bars that show what you get if you subtract off NE2001, YMW16, and/or some halo contribution
    \item BPT diagram with all FRB host galaxies available with standardized colors
    \item a "unified theory" picture for a magnetar engine showing different proposed sites of the FRB emission and the type of emission
    \item an updated/cleaner version of the R3 periodicity plot, ask Dongzi for this (which I think she will be happy to do) and give her direct credit
    \item the "transient parameter space" plot but zoom in to the microseconds to seconds regime and label individual FRBs, SGRs, Crab, etc. and different colors for magnetic powered pulsars, SGRs etc.
    \item a diagram/infographic illustrating the different propagation effects like Faraday rotation, DM, scattering with some annotation describing what they are physically probing and how we can use each one to answer interesting science questions
    \item a 3D volume plot with distances to known FRBs? (Jason: is this the one you were thinking of plotting in supergalactic coordinates?)

\end{itemize}
\end{itemize}
\bigskip 

\textbf{Friday 21 August}
\begin{itemize}
    \item Contact the editor to see if there's a budget for getting the diagrams commissioned
    \item Change document title to ``Fast Radio Bursts: An Addendum''
\end{itemize}
\bigskip 

\textbf{Friday 28 August}
\begin{itemize}
    \item Check with Luigina about the formal invitation for the review
    \item Observational results punchlines:
    \begin{itemize}
        \item Evidence for some FRB-SGR connection
        \item Host galaxy distribution suggests they can'ta ll be young magnetars
        \item Can't just do it all with a single canonical source
        \item If SGR 1935 is representative then you might as well forget about X-ray detections. But still no info about optical flashes. (This maybe feeds more into future observations)
        \item Mention that we have so many instruments searching now -> from a cake pan to a 500-m dish
    \end{itemize}
    \item Figure idea: Number of papers over time that mention ``FRBs'', cumulative plot annotated with important events (similar to Vikram's talk at FRB2019)
    \item Table idea: Similar to Shivani's table in a recent paper with observations, classes of theories with a \checkmark or X 
    \item Figure idea: Variation of parameters (FoV, scattering, etc.) as a function of observing frequency
\end{itemize}
\bigskip

\textbf{Friday 4 September}
\begin{itemize}
    \item 2 -- 3 main takeaways from each section
    \item \textbf{Introduction}
    \begin{itemize}
        \item Punchline: so much progress in the past 2 years
        \item Motivation for this review. Why now? Why so soon after the previous one?
        \item Figures: updated population distributions, number of papers over time, Figure from CHIME with repeaters and bursts over time?
    \end{itemize}
    \item \textbf{Recent observational breakthroughs}
    \begin{itemize}
        \item FRB--SGR connection for some sources
        \item Young magnetars can't explain it all (host galaxies)
        \item Diversity in the FRB population
        \item Exciting big results -- periodicity, polarization, narrow band 
    \end{itemize}
    \item \textbf{Motivation for continued observations}
    \begin{itemize}
        \item Archetypes from CHIME sample motivate what we look for next (analogy with SN Ia)
        \item Parameter space diagram showing where we have coverage
        \item Discussion about what we may have missed because it's too bright (maybe need a telescope like mega-STARE or mini-CHIME)
        \item How we can further constrain the SGR link
        \item We may not ever get one clear answer. But keep in mind what we could still use them for (Section 5)
    \end{itemize}
    \item \textbf{Constraints on theory}
    \begin{itemize}
        \item Host galaxies and locations in them
        \item Wide range of RMs in repeater population
        \item Periodicity and theories specifically related to this. How could future FRB observations constrain this further? What observations would break the theory degeneracy?
        \item Multi-wavelength observations
        \item What we see as the important theoretical developments recently and ahead. Predictive power to explain: multi-wavelength emission, shortest FRB durations, periodicity on many timescales, etc.
    \end{itemize}
    \item \textbf{FRB use cases}
    \begin{itemize}
        \item Parallel with pulsars. Don't understand them, but use them for many interesting applications.
        \item Keep a positive tone about their future uses
    \end{itemize}
    \item \textbf{Future prospects}
    \begin{itemize}
        \item Future of optical short transient surveys
        \item Predictions + reflections on past predictions
    \end{itemize}
\end{itemize} 
\bigskip 

\textbf{Friday 11 September}
\begin{itemize}
    \item Where to put the Macquart relation equation? In the introduction? In Section 5?
    \begin{itemize}
        \item Maybe just mention it in Section 1 to motivate the review?
    \end{itemize}
    \item Dunc's updates
    \begin{itemize}
        \item Start off writing a few paragraphs to get a feel
        \item Population plots might have to wait until CHIME catalogue. And Aitoff projection here might be nice
        \item Put things in broader context (astronomy, transients, previous review)
        \item \textbf{Emily:} Ping Vicky, Ziggy, Alex, others? about the timeline for the catalogue paper. Ask on behalf of the review
        \item \textit{Figure idea:} 2-D histogram of width and DM? See if this makes visual sense
    \end{itemize}
    \item Jason's updates
    \begin{itemize}
        \item Putting in some starter text with some informal language for what we want to cover here
        \item Section 2: why these new results are impactful and important
    \end{itemize}
    \item Emily's updates
    \begin{itemize}
        \item Section 4: Presenting this as a series of observations and what theories they constrain
        \item More focus on progenitor systems than emission mechanisms in this review since that may remain a total unknown for the near future
        \item But also how our observational effects can cause noise or make FRBs ineffective probes (maybe this belongs in Section 5)
    \end{itemize}
    \item Section 4 discussion
    \begin{itemize}
        \item Dunc wonders: does the intrinsic, resolved widths of FRBs make GPs a bit of a nonstarter? Jason: Not necessarily, since these have some structure that could be summed to produce a wider pulse
        \item One interesting observation that hasn't been well addressed by theories: the huge range of observed widths of FRBs basically from microseconds to 10s of ms. Also range of widths within a specific burst from different sub-pulses
        \item good to make this section a little provocative. Poke the theorists
        \item Maybe a list of observed properties that there are currently \textbf{no theories} to explain
    \end{itemize}
\end{itemize}
\bigskip 

\textbf{Friday 18 September}
\begin{itemize}
    \item Perhaps a new title that's more evocative? This should be fine. It just has to be clear that it follows on from the previous one.
    \item Emily: List of observations that theorists haven't explained
    \begin{itemize}
        \item Make this provocative and a bit confrontational
    \end{itemize}
    \item Dunc: Wants ot just set aside some time to put $\sim$a page of rough text in the intro so that words are on the page
    \begin{itemize}
        \item Is there any good way to discuss the limits across different wavelengths? Not just sensitivity, but maybe also timescales as well?
        \item Putting FRB developments in the context of other developments -- GWs, Optical, X-ray, etc.
    \end{itemize}
    \item Jason: started writing some text for Section 2, we can have a look
\end{itemize}

\bigskip

\textbf{Friday 9 October}
\begin{itemize}
    \item Jason
    \begin{itemize}
        \item Working on Section 2, working under labeled headings
        \item next one: multiwavelength observations and constraints, i.e. Younes et al paper with local X-ray timing solution 
        \item Considering the FAST luminosity distribution. What is the minimum energy of an FRB? Contrast with the bursts from the SGR which seem to have similar rates at very different luminosities 
        \item \textbf{We need a timeline on the FAST paper. Dunc says it should be submitted in the next $\sim$week. Update on this next time}
    \end{itemize}
    \item Dunc
    \begin{itemize}
        \item Moved on to Section 5. Putting together all the main papers he wants to talk about
        \item Suggestion to include the Takahashi paper from the arXiv this past week 
    \end{itemize}
    \item Emily
    \begin{itemize}
        \item Are there any models that we can really say are ruled out? I don't think this section is going to end up being very \textit{conclusive} but could just be more elaborative
        \item Are shock models still possible? The varried timescales, short repetition times, PA swings, etc. from some repeaters make this probably unlikely
        \item This would require a dramatic injection of energy and on very extreme timescales (short)
        \item If this is the case you would need crustal cracking or something and this needs so much energy
        \item Pawan and Maxim both don't really see how it can work
        \item Plus the issue of getting emission from a tiny tiny region of a huge shock front
        \item Emily probably needs to think about this more. Maybe have a chat with Pawan or Maxim to walk through it.
    \end{itemize}
    \item The 28 April SGR Event
    \begin{itemize}
        \item Do we call this a Galactic FRB?
        \item Call it what it is... a "candidate FRB"
        \item Maybe a table of pros and cons for calling it an FRB or maybe a subsection called "Is the burst of 28 April 2020 an FRB?"
        \item Emily would like to see this as its own topic or subsection so it's easy to find. Jason has already started on this a bit but we may want to separate it out
    \end{itemize}
    \item Next meeting 23 October at our normal time.
\end{itemize}


\end{comment}

